Unitarity, BRST Symmetry and Ward Identities in Orbifold Gauge Theories

We discuss the use of BRST symmetry and the resulting Ward identities for orbifold gauge theories as consistency checks in an arbitrary number of dimensions. We verify that both the usual orbifold symmetry breaking and the recently proposed Higgsless symmetry breaking are consistent with the nilpotency of the BRST transformation. Imposing the Ward identities resulting from the BRST symmetry on the 4-point functions of theory, we obtain relations on the coupling constants that are shown to be equivalent to the conditions for tree level unitarity. We present the complete set of these sum rules also for inelastic scattering and discuss applications to 6-dimensional models and to incomplete matter multiplets on orbifold fixed points.

==> srpics10.tex <==
% srpics.t10 -- generated from srpics.mp
\fmfL(-1.37738,14.6018,rb){$\vec n$}%
\fmfL(16.37738,14.6018,lb){$\vec m$}%
\fmfL(-1.37738,0.3982,rt){$\vec n$}%
\fmfL(16.37738,0.3982,lt){$\vec m$}%


==> srpics11.tex <==
% srpics.t11 -- generated from srpics.mp
\fmfL(7.89122,10.00002,r){$\nofrac {\vec k_+}{\vec k_-}$}%
\fmfL(-1.64667,19.31721,rb){$\vec n$}%
\fmfL(21.64667,19.31721,lb){$\vec m$}%
\fmfL(-1.64667,0.68279,rt){$\vec n$}%
\fmfL(21.64667,0.68279,lt){$\vec m$}%


==> srpics12.tex <==
% srpics.t12 -- generated from srpics.mp
\fmfL(7.89122,10.00002,r){$\nofrac {\vec k_+}{\vec k_-}$}%
\fmfL(-1.64667,19.31721,rb){$\vec n$}%
\fmfL(21.64667,19.31721,lb){$\vec m$}%
\fmfL(-1.64667,0.68279,rt){$\vec n$}%
\fmfL(21.64667,0.68279,lt){$\vec m$}%


==> srpics13.tex <==
% srpics.t13 -- generated from srpics.mp
\fmfL(10.00008,7.89122,t){$\gamma $}%
\fmfL(22.10876,17.99988,l){$\alpha $}%
\fmfL(22.10876,2.00012,l){$\beta $}%


==> srpics14.tex <==
% srpics.t14 -- generated from srpics.mp
\fmfL(22.10876,17.99988,l){$\alpha $}%
\fmfL(22.10876,2.00012,l){$\beta $}%


==> srpics15.tex <==
% srpics.t15 -- generated from srpics.mp
\fmfL(22.10876,17.99988,l){$\alpha $}%
\fmfL(22.10876,2.00012,l){$\beta $}%


==> srpics16.tex <==
% srpics.t16 -- generated from srpics.mp
\fmfL(10.00008,7.89122,t){$\gamma $}%
\fmfL(21.64667,19.31721,lb){$\hat \alpha $}%
\fmfL(21.64667,0.68279,lt){$\hat \beta $}%


==> srpics24.tex <==
% srpics.t24 -- generated from srpics.mp
\fmfL(2.97603,4.59561,rb){$f_j$}%
\fmfL(17.02397,15.40439,lt){$W_b$}%
\fmfL(2.97603,15.40439,rt){$f_i$}%


==> srpics25.tex <==
% srpics.t25 -- generated from srpics.mp
\fmfL(2.97603,4.59561,rb){$W_b$}%
\fmfL(17.02397,4.59561,lb){$H_i$}%
\fmfL(17.02397,15.40439,lt){$H_j$}%


==> srpics26.tex <==
% srpics.t26 -- generated from srpics.mp
\fmfL(2.97603,4.59561,rb){$f_j$}%
\fmfL(17.02397,15.40439,lt){$H_h$}%
\fmfL(2.97603,15.40439,rt){$f_i$}%


==> srpics27.tex <==
% srpics.t27 -- generated from srpics.mp
\fmfL(2.97603,4.59561,rb){$f_j$}%
\fmfL(2.97603,15.40439,rt){$f_i$}%


==> srpics28.tex <==
% srpics.t28 -- generated from srpics.mp
\fmfL(2.97603,15.40439,rt){$H_i$}%
\fmfL(17.02397,4.59561,lb){$W_b$}%
\fmfL(17.02397,15.40439,lt){$W_c$}%


==> srpics29.tex <==
% srpics.t29 -- generated from srpics.mp
\fmfL(2.97603,15.40439,rt){$W_c$}%
\fmfL(17.02397,15.40439,lt){$W_d$}%


==> srpics3.tex <==
% srpics.t3 -- generated from srpics.mp
\fmfL(10.00008,7.89122,t){$\nofrac {0}{2\vec n}$}%
\fmfL(-1.64667,19.31721,rb){$\vec n$}%
\fmfL(21.64667,19.31721,lb){$\vec n$}%
\fmfL(-1.64667,0.68279,rt){$\vec n$}%
\fmfL(21.64667,0.68279,lt){$\vec n$}%


==> srpics31.tex <==
% srpics.t31 -- generated from srpics.mp
\fmfL(2.97603,15.40439,rt){$H_i$}%
\fmfL(17.02397,4.59561,lb){$H_k$}%
\fmfL(17.02397,15.40439,lt){$H_j$}%


==> srpics32.tex <==
% srpics.t32 -- generated from srpics.mp
\fmfL(2.97603,15.40439,rt){$H_i$}%
\fmfL(17.02397,15.40439,lt){$H_j$}%


==> srpics33.tex <==
% srpics.t33 -- generated from srpics.mp
\fmfL(2.97603,15.40439,rt){$H_i$}%


==> srpics4.tex <==
% srpics.t4 -- generated from srpics.mp
\fmfL(7.89122,10.00002,r){$\nofrac {0}{2\vec n}$}%
\fmfL(-1.64667,19.31721,rb){$\vec n$}%
\fmfL(21.64667,19.31721,lb){$\vec n$}%
\fmfL(-1.64667,0.68279,rt){$\vec n$}%
\fmfL(21.64667,0.68279,lt){$\vec n$}%


==> srpics5.tex <==
% srpics.t5 -- generated from srpics.mp
\fmfL(7.89122,10.00002,r){$\nofrac {0}{2\vec n}$}%
\fmfL(-1.64667,19.31721,rb){$\vec n$}%
\fmfL(21.64667,19.31721,lb){$\vec n$}%
\fmfL(-1.64667,0.68279,rt){$\vec n$}%
\fmfL(21.64667,0.68279,lt){$\vec n$}%


==> srpics6.tex <==
% srpics.t6 -- generated from srpics.mp
\fmfL(-1.37738,14.6018,rb){$n$}%
\fmfL(16.37738,14.6018,lb){$n$}%
\fmfL(-1.37738,0.3982,rt){$n$}%
\fmfL(16.37738,0.3982,lt){$n$}%


==> srpics7.tex <==
% srpics.t7 -- generated from srpics.mp
\fmfL(10.00008,7.89122,t){0}%
\fmfL(-1.64667,19.31721,rb){$\vec n$}%
\fmfL(21.64667,19.31721,lb){$\vec m$}%
\fmfL(-1.64667,0.68279,rt){$\vec n$}%
\fmfL(21.64667,0.68279,lt){$\vec m$}%


==> srpics8.tex <==
% srpics.t8 -- generated from srpics.mp
\fmfL(7.89122,10.00002,r){$\nofrac {\vec k_+}{\vec k_-}$}%
\fmfL(-1.64667,19.31721,rb){$\vec n$}%
\fmfL(21.64667,19.31721,lb){$\vec m$}%
\fmfL(-1.64667,0.68279,rt){$\vec n$}%
\fmfL(21.64667,0.68279,lt){$\vec m$}%


==> srpics9.tex <==
% srpics.t9 -- generated from srpics.mp
\fmfL(7.89122,10.00002,r){$\nofrac {\vec k_+}{\vec k_-}$}%
\fmfL(-1.64667,19.31721,rb){$\vec n$}%
\fmfL(21.64667,19.31721,lb){$\vec m$}%
\fmfL(-1.64667,0.68279,rt){$\vec n$}%
\fmfL(21.64667,0.68279,lt){$\vec m$}%

